Specula: Scaling formal specifications for autonomous model checking of system code

Specula is a push-button agentic system that generates high-quality formal specifications for large, complex system code and uses the specifications for highly effective model checking and bug finding. Specula employs large language model (LLM) based coding agents to autonomously develop TLA+ specifications, including invariants that describe correctness properties of the target system and formal models that describe the system implementation with the right level of abstractions. Specula is fully autonomous and thus eliminates the barrier of applying formal methods to real-world system code (as in traditional human-centric approaches). Meanwhile, Specula addresses limitations of LLM-driven techniques like reward hacking and hallucinations through self-evolving loops that iteratively improve specification quality by enabling the agents to deepen their understanding of system code and its behaviors. We have used Specula to check 48 open-source system projects; Specula found 249 bugs including many deep bugs that are hard to find by existing approaches. Specula has been used by several companies and is maintained at https://github.com/specula-org/Specula.

==> code/etcd-election-safety.tex <==
\begin{minted}[escapeinside=\%\%,breaklines,breakanywhere,breakautoindent]{text}
ElectionSafety %\PYG{o}{==}%
    %\PYG{o}{\symbol{92}A}% s1, s2 %\PYG{o}{\symbol{92}in}% Server :
        (state%\PYG{o}{[}%s1%\PYG{o}{]}% %\PYG{o}{=}% Leader %\PYG{o}{/\symbol{92}}% state%\PYG{o}{[}%s2%\PYG{o}{]}% %\PYG{o}{=}% Leader
            %\PYG{o}{/\symbol{92}}% currentTerm%\PYG{o}{[}%s1%\PYG{o}{]}% %\PYG{o}{=}% currentTerm%\PYG{o}{[}%s2%\PYG{o}{]}%)
        %\PYG{o}{=}%%\PYG{o}{>}% s1 %\PYG{o}{=}% s2
\end{minted}


==> code/hashiraft-nophantomcontact.tex <==
\begin{minted}[escapeinside=\%\%,breaklines,breakanywhere,breakautoindent]{text}
%\PYG{c+c1}{\symbol{92}* A lease counts a follower only while its term is not ahead}%
NoPhantomContact %\PYG{o}{==}%
    %\PYG{o}{\symbol{92}A}% s %\PYG{o}{\symbol{92}in}% Server :
        state%\PYG{o}{[}%s%\PYG{o}{]}% %\PYG{o}{=}% Leader %\PYG{o}{=}%%\PYG{o}{>}%
            %\PYG{o}{\symbol{92}A}% f %\PYG{o}{\symbol{92}in}% leaseContact%\PYG{o}{[}%s%\PYG{o}{]}% :
                currentTerm%\PYG{o}{[}%f%\PYG{o}{]}% %\PYG{o}{<}%%\PYG{o}{=}% currentTerm%\PYG{o}{[}%s%\PYG{o}{]}%
\end{minted}


==> code/papaya-spec.tex <==
\begin{minted}[escapeinside=\%\%,breaklines,breakanywhere,breakautoindent]{text}
%\PYG{c+c1}{\symbol{92}* snippet of spec translated from mod.rs lines 6-9}%
%\PYG{n+nf}{AbortResize}%(tid, srcT, abortedT) %\PYG{o}{==}% %\PYG{c+c1}{\symbol{92}* an action}%
  %\PYG{c+c1}{\symbol{92}* ...}%
  %\PYG{o}{/\symbol{92}}% parked%\PYG{o}{'}% %\PYG{o}{=}% %\PYG{o}{[}%th %\PYG{o}{\symbol{92}in}% Thread %\PYG{o}{|->}%
     %\PYG{c+c1}{\symbol{92}* BUG: srcT should be abortedT}%
     %\PYG{k}{IF}% parked%\PYG{o}{[}%th%\PYG{o}{]}% %\PYG{o}{/=}% NULL
        %\PYG{o}{/\symbol{92}}% parked%\PYG{o}{[}%th%\PYG{o}{]}%.table %\PYG{o}{=}% srcT
     %\PYG{k}{THEN}% NULL %\PYG{k}{ELSE}% parked%\PYG{o}{[}%th%\PYG{o}{]}%%\PYG{o}{]}%

NoParkedOnAborted %\PYG{o}{==}% %\PYG{c+c1}{\symbol{92}* the violated invariant}%
    %\PYG{o}{\symbol{92}A}% tid %\PYG{o}{\symbol{92}in}% Thread :
        parked%\PYG{o}{[}%tid%\PYG{o}{]}% %\PYG{o}{/=}% NULL %\PYG{o}{=}%%\PYG{o}{>}%
        resizeStatus%\PYG{o}{[}%parked%\PYG{o}{[}%tid%\PYG{o}{]}%.table%\PYG{o}{]}% %\PYG{o}{/=}% ABORTED
\end{minted}


==> code/sofa-vote-durable.tex <==
\begin{minted}[escapeinside=\%\%,breaklines,breakanywhere,breakautoindent]{text}
VoteIsDurable %\PYG{o}{==}%
    %\PYG{o}{\symbol{92}A}% m %\PYG{o}{\symbol{92}in}% messages :
        (m.mtype %\PYG{o}{=}% RequestVoteResp %\PYG{o}{/\symbol{92}}% m.granted) %\PYG{o}{=}%%\PYG{o}{>}%
            %\PYG{o}{/\symbol{92}}% durable%\PYG{o}{[}%m.src%\PYG{o}{]}%.term %\PYG{o}{=}% m.mterm
            %\PYG{o}{/\symbol{92}}% durable%\PYG{o}{[}%m.src%\PYG{o}{]}%.vote %\PYG{o}{=}% m.dst
\end{minted}


==> sections/understanding.tex <==
\subsection{Understanding system artifacts}
\label{sec:design-system-understanding}

\specula makes modeling decisions of a given system 
    based on its understanding of the system artifact 
    (typically the software repository of the system project).
The artifact often includes source code (including test code), 
    revision history,
    reported issues, pull requests, 
    and documents.
\specula analyzes
    the artifact and generates a structured
    document, termed {\it modeling plan},
    which is used to guide the specification generation.
Figure~\ref{fig:scylla-brief} exemplifies
    the modeling plan \specula generates
    for ScyllaDB's Raft library~\cite{}.

A model plan includes a system description, 
    invariants,
    faults that should be tolerated by the system.
% The goal of system understanding is to convert repository evidence into project-specific modeling decisions 
% before any \tla spec is written.
% A spec that supports meaningful model checking of the system must hold four properties at once: 
% (1) it must preserve the implementation semantics that make a target failure visible, 
% (2) choose action boundaries and fault assumptions under which the failure can be reached, 
% (3) carry invariants that the failure violates, and 
% (4) leave model checking a search space small enough to explore within budget.
% Satisfying these four together requires project-specific knowledge: 
% which mechanisms in this codebase may hide subtle bugs, 
% which fault assumptions and action sequences may expose them, and which abstractions may remain safe.
% An AI agent invoked on an unfamiliar codebase does not have this knowledge.
% \specula's first step builds it from repository evidence.
The analysis is done by instructing AI agents to {\it summarize}
(1) system constructions and abstractions 
    in the form of modules, actions, and their concurrency,
(2) fault models and invariants,
and (3) different granularities of modeling the system~\cite{ouyang2025remix}.
The detailed prompt can be found in Appendix~\ref{sec:}.
In our experience, state-of-the-art agents have strong capabilities of 
    summarization and excel in this task.

% \begin{itemize}[leftmargin=*]
%  \item \textbf{Structural reconnaissance.} 
%        Map modules, concurrency model, and atomicity boundaries, 
%        and classify the system into a category such as distributed (message-passing) or concurrent (lock-free).
%    \item \textbf{Repository mining.} Mine commits, issues, pull requests, and code comments to identify the invariants worth checking and the fault setups that may violate them.
%    \item \textbf{Implementation analysis.} With the invariants and fault setups in hand, read the implicated code paths to decide which implementation details must be modeled and which can be abstracted. 
%    An implementation detail enters the model only when it may affect whether one of the scenario's invariants is violated.
% \end{itemize}

A modeling plan also includes a set of scenarios that
    \specula would focus on in model checking (see \S\ref{sec:specgen}).
Given the vast search space, these scenarios
    help \specula focus on checking the system's
    most significant and potentially vulnerable behaviors, 
    increasing the likelihood of detecting faults that may only manifest under specific conditions.
Unlike prior work that relies on developers to provide the scenarios~\cite{Li:nsdi:2026,need_more},
    \specula automatically generates scenarios by reading code,
    documents, comments, reported issues, etc.
\specula enforces the AI agent to provide {\it evidence} when generating a scenario---specific commits, issues, comments, 
    or other information that describes the scenario---making 
    the scenario auditable and minimizing hallucination.
Each scenario lists the target module in the system 
    and a proposal of modeling the scenario.

\begin{figure}[t]
    \centering
%    \rule{\linewidth}{0.4pt}\par
    \inputminted{yaml}{code/scylla-scenario.md}
%    \rule{\linewidth}{0.4pt}\par
    \caption{A simplified modeling plan produced by \specula's analysis for ScyllaDB's Raft library.}
    \label{fig:scylla-brief}
\end{figure}

Figure~\ref{fig:scylla-brief} shows a scenario of joint-consensus reconfiguration during voter demotion
    in ScyllaDB, where a node is voter in the previous configuration but non-voter in the current one.
\specula creates this scenario because it observes that (1) the related code 
    has been changed by multiple fixes and (2) the fixes are inconsistent in diferent code snippets.
% This pattern may violate , so the area enters the modeling proposal.
In fact, this scenario enabled \specula to discover a new bug that stalls a read barrier during 
    voter demotion, which violates the \textsf{ReadBarrierProgress} invariant.
We have reported the bug which has been fixed in ScyllaDB.   
% PR~\#29226.

\TODO{@tianyin will write some summary sentences: (1) emphasize why the evidence-based approach 
    makes sense, and (2) emphasize that the approach accommodates the evolution of the system
    as the specification generation is cheap.}

% admits implementation details based on whether they may affect those invariants, not by excluding utility code wholesale.
% For example, hashes are normally excluded from the spec as pure utilities, but papaya is the exception.
% Papaya stores hash bits in a per-slot meta byte, and the order in which this byte and the entry pointer are published can leave a \texttt{get} returning ``not found'' for a key still present in the table.
% The meta/entry publication semantics therefore enter the model; the hash function itself stays out.


